Causal Responder Detection

We introduce the causal responders detection (CARD), a novel method for responder analysis that identifies treated subjects who significantly respond to a treatment. Leveraging recent advances in conformal prediction, CARD employs machine learning techniques to accurately identify responders while controlling the false discovery rate in finite sample sizes. Additionally, we incorporate a propensity score adjustment to mitigate bias arising from non-random treatment allocation, enhancing the robustness of our method in observational settings. Simulation studies demonstrate that CARD effectively detects responders with high power in diverse scenarios.

==> misc/junk.tex <==

\subsection{Scorer}

A key difference in the setting of the suggested 
We suggest a tree-scorer similar to causal-forest. The goal 

Suppose we are given access to $\mathcal{A}$, a set of all $x$s for which the distribution of the treated and untreated differs. 

$$\mathcal{A} = \{x: P_{Y|X=x, t=1} \neq P_{Y|X = x, t = 0} \}.$$

A natural approach for testing the hypothesis in Eq. \ref{eq:hypo_test} would be estimating $P_{Y| T = 0, x \in \mathcal{A}}$ and rejecting the hypothesis for $Y_i(1)$ that appear extreme according to the estimated distribution. Unfortunately, $\mathcal{A}$ is typically unknown and must be estimated from the available data. 

To address this challenge, we propose the Distribution Tree (DT) algorithm. Our approach mirrors the principles of a Causal Tree, wherein the data is recursively partitioned on $X$ to maximize the overall $\mathrm{Loss}_y$ across partitions until certain stopping criteria, such as reaching a maximum tree depth or convergence of loss, are met. The loss $\mathrm{Loss}_y$ is a function measuring the difference of the distribution between $(y_i, t_i = 1)$ and $(y_i, t_i = 0)$. This framework mandates that the final splits are determined based on $y$, yet it remains flexible to accommodate various difference functions beyond average differences.

Let $L$ define a set of observations that adhere to a specific condition on $x$ or $y$ (i.e., a leaf of a tree), 

\begin{equation} \label{eq:tree_loss}
\mathrm{Loss}_x(L) = w_l \mathrm{Loss}_y(f_y(L_l))  + w_r \mathrm{Loss}_y(f_y(L_r)).
\end{equation}

where $L_l$ and $L_r$ are a partition of $L$ such there is some $j$ and $\xi$ that $L_l = \{i: i \in L, x_{i, j} \leq \xi\} $ and $L_r = \{i: i \in L, x_{i, j} > \xi\}$. $w_l, w_r$ the weights, which can be a function of the leaf-size. Finally, 
$f_y$ is some function of only the response, aimed at discriminating between $Y(0)$ and $Y(1)$. Since the choice of $f_y$ and $\mathrm{Loss}_y$ are affected by the testing procedure, we will delay the discussion of their choices until after describing the testing procedure.  

\subsection{Testing Procedure}

Once the partitions are determined, our objective is to test Eq. \ref{eq:hypo_test} either within specific partitions or across multiple partitions. However, directly estimating $P_{Y| x \in \mathcal{A}, T = 0}$ is not appropriate because this estimation was used in determining the partitions. Therefore, reusing it for testing would result in a liberal testing procedure. 

To address this issue of selection bias, we adopt a strategy similar to AdaDetect [CITE]. We split the untreated sample $\mathcal{I}_0 = \{i: t_i = 0 \}$ into a knockoff sample $\mathcal{I}_{ko}$ and the remaining untreated observations, $\mathcal{I}_0^*$. We then apply a scoring algorithm (such as DT or an ensemble of DTs) to discriminate between $\mathcal{I}_1 \cup \mathcal{I}_{ko}$ and $\mathcal{I}_0^*$. 

Let $s(x_i, y_i)$ be the resulting score according to the algorithm, and denote by $\mathcal{S}_{ko} = {s(x_i, y_i): i \in \mathcal{I}_{ko} }$, and similarly $\mathcal{S}_1$. Since both sets of observations $\mathcal{I}_{ko}$ and $\mathcal{I}_1$ underwent the same selection process, under the null hypothesis, the scores in $\mathcal{S}_{ko}$ and $\mathcal{S}_1$ are exchangeable. This exchangeability of scores implies that the p-values according to Eq. \ref{eq:unweighted_adadetect_pval} are valid for testing the hypothesis Eq. \ref{eq:hypo_test}.

\subsection{Choice of $\mathrm{Loss}_y$ and $f_y$}

The choice of $\mathrm{Loss}_y$ and $f_y$ is crucial in the testing procedure. Since the goal is to discriminate the between $y(0)$ and $y(1)$ natural candidates for $\mathrm{Loss}_y$ and $f_y$ are the Gini impurity measure, and a classification tree respectively. The score function, $s$, is the proportion of treated in the terminal leaf of the observation. 

However, there are a few drawbacks in the use of the classification tree, first, classification trees treat both classes symmetrically, in our case however the interest lies only on $\mathcal{I}_1^*$. Second, the scores given by the tree are constant across the terminal leaves. Since the testing procedure involves comparison of the scores of the knockoffs and treated group, a score function which gives a higher score the more extreme the response is will increase power. 

Our suggested approach is to quantify the unlikeness of an observation in a specific leaf using a pseudo p-value, and to summarise the loss over multiple observation by summing the log of the these p-values. P-values often used to measure the extremeness of an observation with respect to a specific distribution. Furthermore, it is a continuous measure which differs as a function of $y$. Finally, we will see that the approaches based on density are pivotal for ensuring double-robustness.  

The pseudo p-value of observation $y_i$ is, $$p_i = p(y_i; L_i) = 2 \times \min \left( \frac{\sum_{j \in L} I(y_i \leq y_j, t_j = 0)}{\sum_{j \in L} I(t_j = 0)}, \frac{\sum_{j \in L} I(y_i \geq y_j, t_j = 0)}{\sum_{j \in L} I(t_j = 0)}   \right),$$

where $L_i$ is the terminal leaf such that $(x_i, y_i, t_i) \in L_i$. The function, $f_y$ is the sum of pseudo p-values logits,  $f(y) = \sum_i \log \frac{p_i}{1 - p_i}$ and $\mathrm{Loss}_y = \sum_{i: t_i = 1} \log(p_i)$. The score, $s$ is the logit of the psuedo p-value. 



\subsection{Causal Knockoffs are Exact in RCT}

The testing procedure described above relies on the fact that $e(x) = c$ ($c$ being some constant), or that $Y(0) \perp X$ under the null hypothesis, otherwise, $\mathcal{S}_{ko}$ and $\mathcal{S}_1$ are not exchangeable. Thus, rejecting Eq. \ref{eq:hypo_test}, could be due to bias cause by the propensity score, inflating the the type I error. 

In the case of randomized control trials (RCT, with perfect compliance) where  $T \not\perp X$, the randomization ensures that $e(x) = c$, and the method can be applied as is ensuring control of the error at exactly the specified rate.

Whenever the propensity score is not constant, $e(x) \neq c$, and $Y(0) \not\perp X$, the suggested procedure is no longer valid. The scores of the knockoff group are no longer exchangeable with the treated observations (under the null). 
Given the propensity score, we define the weights, $w_i^* = \frac{e(x)}{1 - e(x)}$, and the weights are $w_i = w_i$

$w_i = \frac{e(x_i)}{\sum_{j \in \mathcal{I}_{ko}} e(x_j) }$, the p-values of the adjusted procedure is,

\begin{equation} \label{eq:weighted_pvalues}
    \mathrm{w-pv}_i = \frac{1}{k+1} + \sum_{j=1}^k  w_j \times I\left(s(x_j, y_j) > s(x_i, y_i)\right).
\end{equation}

The next lemma proves the validity of the adjustment, 


\begin{lemma}
    Under the null hypothesis (Eq. \ref{eq:hypo_test}), the weighted p-values (Eq. \ref{eq:weighted_pvalues}) control the type I error at level $\alpha$, 

    $$ \bb{P}(w-pv_i < \alpha) \geq \alpha .$$
\end{lemma}





